Malaysian English News Decoded: A Linguistic Resource for Named Entity and Relation Extraction

Standard English and Malaysian English exhibit notable differences, posing challenges for natural language processing (NLP) tasks on Malaysian English. Unfortunately, most of the existing datasets are mainly based on standard English and therefore inadequate for improving NLP tasks in Malaysian English. An experiment using state-of-the-art Named Entity Recognition (NER) solutions on Malaysian English news articles highlights that they cannot handle morphosyntactic variations in Malaysian English. To the best of our knowledge, there is no annotated dataset available to improvise the model. To address these issues, we constructed a Malaysian English News (MEN) dataset, which contains 200 news articles that are manually annotated with entities and relations. We then fine-tuned the spaCy NER tool and validated that having a dataset tailor-made for Malaysian English could improve the performance of NER in Malaysian English significantly. This paper presents our effort in the data acquisition, annotation methodology, and thorough analysis of the annotated dataset. To validate the quality of the annotation, inter-annotator agreement was used, followed by adjudication of disagreements by a subject matter expert. Upon completion of these tasks, we managed to develop a dataset with 6,061 entities and 3,268 relation instances. Finally, we discuss on spaCy fine-tuning setup and analysis on the NER performance. This unique dataset will contribute significantly to the advancement of NLP research in Malaysian English, allowing researchers to accelerate their progress, particularly in NER and relation extraction. The dataset and annotation guideline has been published on Github.

==> chapters/experiment-result.tex <==
\section{Experiment Result and Analysis}
\label{sec: experiment}
% \begin{figure*}[h]
%     \centering
%     \includegraphics[height=\textheight,width=\textwidth,keepaspectratio]{figures/Barchart-Evaluation-BERT-NER-FineTune.png}
%     \caption{The precision, recall and F1-Score calculated based on validation set.}
%     \label{fig:Barchart-Evaluation-NER-FineTune}
% \end{figure*}

% \begin{figure*}[h] 
%     \centering
%     \includegraphics[height=\textheight,width=\textwidth,keepaspectratio]{figures/Barchart-Evaluation-spaCy-NER-FineTune.png}
%     \caption{The precision, recall and F1-Score calculated based on validation set.}
%     \label{fig:Barchart-Evaluation-NER-spacy-FineTune}
% \end{figure*}

\subsection{Further Pre-training Language Model}
\label{ssec: fp-result-and-analysis}

\subsubsection{PLM Training Evaluation}
\label{ssec: bert-train-loss}
Figure \ref{fig:Training-Loss-3FP} (in Appendix \ref{appendix:Training-Loss}) visualize the training loss across 30 epochs for three pre-trained language models (named MENmBERT-FP, MENBERT-FP, and MENBERT-SC), while Figure \ref{fig:Training-Loss-2FP} is only to compare the training loss between two pre-trained language model (named MENmBERT-FP, and MENBERT-FP). Based on Figure \ref{fig:Training-Loss-3FP} (in Appendix \ref{appendix:Training-Loss}), MENBERT-SC has the highest training loss compared to other two further pre-trained model. Observe that the loss values for MENBERT-FP and MENmBERT-FP are quite close at most epochs. This indicates that these two models are performing similarly during training. As overall we can observe that all three models exhibits steady decrease in loss as training progresses. Based on the training loss, it shows that MENmBERT-FP, MENBERT-FP are better performing in the train corpus compared to MENBERT-SC. Considering this in mind, we will fine-tune the pre-trained model to identify how good are they performing in downstream task like NER. In Section \ref{ssec: ft-ptm} we have discussed on the performance of fine-tuned model. 

\subsubsection{Model Masking Evaluation}
\label{ssec: bert-masked-language}
To evaluate performance of pre-trained language model, we will fine-tune the model to downstream task. However \citep{Salazar_2020, kauf2023better} has proposed "pseudo-log-likelihood" score that computed by masking tokens one by one. The score is computed by summing the log-losses at the different masked positions. However, we are more interested to observe how well the model uncover the mask for new sentences. To understand that, we have selected 20 new sentences from Malaysian English news portal and random apply <MASK> for tokens that exhibit morphosyntactic adaptation. Each sentence will then be passed to pre-trained model and require it to predict the masked token. 
For each pre-trained model we will calculate the ratio of sentence that has correctly predicted the masked token. This ratio will allow us to understand how pre-trained models are performing. We have set bert-based-cased and ber-base-multilingual-cased has been used as baseline for this evaluation. Based on the Table \ref{tab:random-mask} (in Appendix \ref{appendix:masking-token}) that presents the result of tokens predicted by different pre-trained BERT model, MENmBERT-FP contributes the highest ratio (45\%) of success. Meanwhile, bert-based-cased and MENBERT-SC has achieved 0\% of success. Here are the findings observed from result in Table \ref{tab:random-mask} (the ordering of the below list is based on the \% of Success):
\begin{enumerate}
    \item MENmBERT-FP: In some cases, the model only able to unmask partial of the tokens. For example, when unmasking token \textit{Gabungan} it predicted as \textit{\#\#bungan}. This could be due to the tokenizer. 
    \item mbert-based-cased: In some cases, the model only able to unmask partial of the tokens. Since mbert-based-cased has been trained with Bahasa Malaysia, it was able to unmask some of the tokens which exhibits compound blend. 
    \item MENBERT-FP: When we compare the performance of MENBERT-FP with bert-based-cased, we can understand further-pretraining are improving the performance of language model. The success ratio of bert-based-cased is 0, and once further pre-trained we able to see there is +10\%.
    \item bert-based-cased: Since bert-based-cased has only been trained with English corpus, it was not able to unmask any tokens with compound blend correctly. 
    \item MENBERT-SC: Based on our observation, MENBERT-SC has produced bad results when unmasking the tokens. Once fine-tune, we will be able to understand better on the performance of the model. 
\end{enumerate}
In Section \ref{ssec: ft-ptm} we have discussed on the performance of pre-trained model once fine-tune them for NER task.  

\subsection{Performance of NER Model}
\label{ssec: ft-result-and-analysis}
In Section \ref{ssec: menbert-fp} we have discussed about the pre-trained model used to fine-tune in downstream task and in Section \ref{ssec: menbert-ft} we have went through the about fine-tuning approach used. 

\subsubsection{Fine-Tune Pre-Trained Model}
\label{ssec: ft-ptm}
\begin{figure}[H]
    \centering
    \includegraphics[height=\textheight,width=0.5\textwidth,keepaspectratio]{figures/Barchart-Evaluation-BERT-NER-FineTune.png}
    \caption{The precision, recall and F1-Score calculated based on validation set.}
    \label{fig:Barchart-Evaluation-NER-FineTune}
\end{figure}
Figure \ref{fig:Barchart-Evaluation-NER-FineTune} shows the comparison of F1-Score among five different pre-trained models. We are trying to identify if the hypothesis discussed in Section \ref{ssec: menbert-intro} can be achieved once fine-tune the pre-trained model. To evaluate the performance of further pre-trained model, we have also fine-tuned pre-trained model (bert-base-cased, and bert-base-multilingual-cased) as baseline. Figure \ref{fig:Barchart-Evaluation-NER-FineTune} shows Precision, Recall, and F1-Score calculate with validation set (referring Table \ref{tab:dataset-split-ft}). Meanwhile in Figure \ref{tab:entity-label-plm} (in Appendix \ref{appendix:entity-label-plm}) we have break down the performance of model based on entity label.

Based on the result, we can observe that MENmBERT-FP has achieved the highest F1-Score (0.831), while MENBERT-SC has achieved the lowest F1-Score (0.316). However, the result in Figure \ref{fig:Barchart-Evaluation-NER-FineTune} shows there is improvement when further pre-train BERT model, and this has shown that our hypothesis (discussed in Section \ref{ssec: menbert-intro}) is valid. Here are few other observation from this experiment:
\begin{enumerate}
    \item MENmBERT-FP (F1-Score is 0.831) has higher F1-Score than mBERT-base-cased (F1-Score is 0.819). We can see there is an improvement of +1.52\%. Although the improvement is not significant, when we analyse the F1-Score based on the Entity Label wise:
    \begin{enumerate}
        \item There is an significant improvement for 6 out of 11 entity labels that are evaluated. 
        \item On average the difference in F1-Score between MENmBERT-FP and mBERT-base-cased is +10\%. 
        \item mBERT-base-cased has only able to achieve on-par F1-Score with MENmBERT-FP for entity label ORGANIZATION. 
    \end{enumerate}
    This in deep observation entity label wise, has proven the performance of MENmBERT-FP is much significant. 
    \item MENBERT-FP (F1-Score is 0.778) has higher F1-Score than bert-based-cased (F1-Score is 0.763) with improvement of +1.94\%. However the F1-Score of still lower than MENmBERT-FP and mBERT-base-cased. We have further investigate the performance based on entity label:
    \begin{enumerate}
        \item MENBERT-FP has only improved the performance of only 7 out of 11 entity labels. 
        \item On average the improvement is only around +2\%.
        \item When compared with MENmBERT-FP, MENBERT-FP able to outperform F1-Score of 4 out of 11 entity labels. This includes entity label PRODUCT, FACILITY, NORP and LAW. 
    \end{enumerate}
    \item MENBERT-SC has not shown any improve in the performance of NER. Our evaluation in Section \ref{ssec: bert-masked-language}, also shows it was not able to unmask the tokens correctly. 
\end{enumerate}
As conclusion, our fine-tuned MENmBERT-FP has achieved highest F1-Score compared to other pre-trained model evaluated in this experiment. 

\subsubsection{Fine-Tune Spacy}
\label{ssec: ft-spacy}
\begin{figure}[H] 
    \centering
    \includegraphics[height=\textheight,width=0.5\textwidth,keepaspectratio]{figures/Barchart-Evaluation-spaCy-NER-FineTune.png}
    \caption{The precision, recall and F1-Score calculated based on validation set.}
    \label{fig:Barchart-Evaluation-NER-spacy-FineTune}
\end{figure}
In Figure \ref{fig:Barchart-Evaluation-NER-spacy-FineTune} we have visualized the performance of spaCy NER component with different type of models. To evaluate the performance of NER model, we have evaluated our validation set on en\_core\_web\_sm, en\_core\_web\_lg, and en\_core\_web\_trf and consider the result as baseline. The result will be compared with spacy-blank, en\_core\_web\_sm-FT, en\_core\_web\_lg-FT, and en\_core\_web\_trf-FT. Meanwhile in Figure \ref{tab:entity-label-spacy} (in Appendix \ref{appendix:entity-label-spacy}) we have break down the performance of model based on entity label.

Based on the result, we can observe that spacy-blank has achieved the highest F1-Score (0.94), while en\_core\_web\_sm-FT has achieved the lowest F1-Score (0.832). On average all the fine-tuned spaCy model has shown an improvement of +230\%, and this improvement is so significant compared to pre-trained language model. If we compared with fine-tuned pre-trained model, the average F1-Score of spaCy (F1-Score is 0.88) model is higher than further pre-trained model (F1-Score is 0.81). In Table \ref{tab:entity-label-spacy} (in Appendix \ref{appendix:entity-label-spacy}), we have break down the performance of model based on entity label:
\begin{enumerate}
    \item Across all the fine-tuned spaCy model, we have seen there is an significant improvement in F1-Score. On average the fine-tuned model (when compared with en\_core\_web\_sm and en\_core\_web\_sm-FT) has achieved F1-Score improvement of +401\%. 
    \item All the three base spaCy models (en\_core\_web\_sm, en\_core\_web\_lg, en\_core\_web\_trf) has obtained F1-Score of 0 for entity label PRODUCT, FACILITY, ROLE, TITLE, LANGUAGE, and WORK\_OF\_ART. It is important to take note that the NER component in spaCy model is trained upon OntoNotes 5.0 \citep{ontonotes-new} dataset, and in MEN-Dataset we have followed 10 out of 12 entity labels in OntoNotes. In that case, apart from the entities labeled as ROLE and TITLE, the base model was expected to predict entities for the remaining entity labels. However, it failed to do so in our experiment.
    \item If we refer back to introduction of Malaysian English (in Section \ref{sec: introduction}), entity label that exhibits morphosyntactic adaptions are TITLE, WORK\_OF\_ART, ORGANIZATION, LOCATION, and FACILITY. For this mention entity label, we can see a significant improvement fine-tuned NER model.  
\end{enumerate}
As conclusion, our custom spaCy NER model called spacy-blank has achieved highest F1-Score compared to other fine-tuned spaCy model. 

\subsection{\textit{Which one is better?}}
\label{ssec: ft-result-and-analysis-conclusion}
In Section \ref{ssec: fp-result-and-analysis}, we discussed the results of the pre-trained language model. In Section \ref{ssec: ft-result-and-analysis}, we compared the results of the fine-tuned model with both the pre-trained language model and spaCy. Based on the fine-tuned result in Section \ref{ssec: ft-result-and-analysis}, we can conclude fine-tuned spaCy NER model named \textbf{spacy-blank} are able to perform better than fine-tuned pre-trained language model. 
However, in the beginning of the research we have discussed about our hypothesis that \textit{having a BERT model with rich language based understanding will improve the performance of NER when fine-tuned them}. The result in \ref{ssec: ft-ptm} proves that our \textbf{hypothesis is valid}, but the performance has not improved significantly. This further pre-trained can be used for other downstream task on Malaysian English. 
